DEJA VU: Continual Model Generalization For Unseen Domains

In real-world applications, deep learning models often run in non-stationary environments where the target data distribution continually shifts over time. There have been numerous domain adaptation (DA) methods in both online and offline modes to improve cross-domain adaptation ability. However, these DA methods typically only provide good performance after a long period of adaptation, and perform poorly on new domains before and during adaptation - in what we call the "Unfamiliar Period", especially when domain shifts happen suddenly and significantly. On the other hand, domain generalization (DG) methods have been proposed to improve the model generalization ability on unadapted domains. However, existing DG works are ineffective for continually changing domains due to severe catastrophic forgetting of learned knowledge. To overcome these limitations of DA and DG in handling the Unfamiliar Period during continual domain shift, we propose RaTP, a framework that focuses on improving models' target domain generalization (TDG) capability, while also achieving effective target domain adaptation (TDA) capability right after training on certain domains and forgetting alleviation (FA) capability on past domains. RaTP includes a training-free data augmentation module to prepare data for TDG, a novel pseudo-labeling mechanism to provide reliable supervision for TDA, and a prototype contrastive alignment algorithm to align different domains for achieving TDG, TDA and FA. Extensive experiments on Digits, PACS, and DomainNet demonstrate that RaTP significantly outperforms state-of-the-art works from Continual DA, Source-Free DA, Test-Time/Online DA, Single DG, Multiple DG and Unified DA&DG in TDG, and achieves comparable TDA and FA capabilities.

==> sections/related_work.tex <==
\section{More Related Work \llv{easy to be diss, better not to put such short paragraph as a sole section.}}
Given that most of domain adaptation and domain generalization studies have already been covered in Section~\ref{Sec_intro}, here we introduce some extra related works. \citet{bai2022temporal} and \citet{nasery2021training} study the model generalization change caused by smooth temporal shifts of data distribution. However, these works cannot handle large distribution changes over time, and they also assume the data that has been seen is available all the time. Another work~\citep{simon2022generalizing} develops a domain generalization framework in a way of class incremental learning in which the target domain is fixed and unchanged. Besides, all the data is well labeled and the source data consists of multiple domains, which is quite different from our problem of interest.

% \textbf{Domain Adaptation} (DA) aims to improve the model performance on an unlabeled target domain when a labeled source domain with covariate shifts is given. There has been quite a few DA studies, \emph{e.g.}, domain discrepancy minimization~\citep{balaji2019normalized}, adversarial training~\citep{wei2021toalign}, and invariant representation learning~\citep{lee2021dranet}. In real world, the target impossibly stays the same all the time, instead, it usually changes over time. To cope with such scenarios, Continual DA~\citep{liu2020learning, rostami2021lifelong} is proposed to achieve best generalization performance across all target domains. However, existing Continuous DA works assume the source domain is always accessible, which is impractical in real world applications. Source-Free DA~\citep{liang2020we, yang2021generalized, qu2022bmd} is proposed recently to relax the demand of source data during adaptation. 
% % SHOT~\citep{liang2020we} designs an effective hypothesis transfer for adapting a trained source model to the target domain. GSFDA~\citep{yang2021generalized} focuses on the learned source knowledge and uses feature clustering for adaptation. BMD~\citep{qu2022bmd} proposes a balanced pseudo labeling method for SHOT and GSFDA. 
% In addition to offline methods, there are some recent studies~\citep{wang2020tent, wang2022continual, iwasawa2021test, panagiotakopoulos2022online} about Test-time or Online DA that can adapt the model by some techniques with small cost. But the improvement is trivial and cannot make the model produce acceptable performance. In short, although the above DA studies can adapt the model to perform better on target domains, the adaptation needs time and requires sufficient target data, making the model cannot be deployed to use before and during adaptation due to poor performance, especially when target domains change suddenly and momentarily.

% \textbf{Domain Generalization} (DG)~\citep{li2021uncertainty, yao2022pcl, zhang2022exact} assumes the target domain is unavailable and unexpected during training, but the objective is to improve the model performance on the target with multiple source domains available. 
% % A number of solutions have been proposed, for example, DSU quantifies the uncertainty of features statistics cross source domains to reduce domain shifts. PCL~\citep{yao2022pcl} proposes a modified contrastive learning algorithm that is beneficial for generalization improvement. EFDM~\citep{zhang2022exact} applies histogram matching to synthesize data samples with diverse styles for improving generalization robustness. 
% More recently, there is a growing interest in achieving DG with only a single source domain available, and well-crafted data augmentations~\citep{wang2021learning, li2021progressive} have been proposed to solve this problem. Besides, there are some works unifying DA and DG~\citep{ghifary2016scatter, motiian2017unified, jin2021style}. In this work, we focus on improving model generalization performance on continually changing target domains. To our best knowledge, there is no prior work that focuses on our problems, though we do notice that some recent studies have begun to study related topics.  

